Cryogenic payloads for the Einstein Telescope -- Baseline design with heat extraction, suspension thermal noise modelling and sensitivity analyses

The Einstein Telescope (ET) is a third generation gravitational wave detector that includes a room-temperature high-frequency (ET-HF) and a cryogenic low-frequency laser interferometer (ET-LF). The cryogenic ET-LF is crucial for exploiting the full scientific potential of ET. We present a new baseline design for the cryogenic payload that is thermally and mechanically consistent and compatible with the design sensitivity curve of ET. The design includes two options for the heat extraction from the marionette, based on a monocrystalline high-conductivity marionette suspension fiber and a thin-wall titanium tube filled with static He-II, respectively. Following a detailed description of the design options and the suspension thermal noise (STN) modelling, we present the sensitivity curves of the two baseline designs, discuss the influence of various design parameters on the sensitivity of ET-LF and conclude with an outlook to future R&D activities.

==> Lennard/TMAR_deltapan_plot.tex <==
%\resizebox{\columnwidth}{!}{%
%\pgfplotsset{width=242.25pt}
\usetikzlibrary{calc}

\begin{tikzpicture}
\pgfplotsset{
    %scale only axis,
    %scaled x ticks=base 10:3,
    xmin=0,
    xmax=5,
    minor x tick num=1,
    grid=major,
    width = 0.431\textwidth,
}

\begin{axis}[
%name = plot,
    width = 0.431\textwidth,
  y axis line style = {KITpurple,line width=0.5pt},
  axis y line*=left,
  %axis x line=none,
  ymin=0, ymax=300,
  ylabel=$\Delta p_\mathrm{He}$ / \SI{}{\milli\bar},
  ylabel style = {KITpurple},
  y tick label style= {KITpurple},
  ytick={0,50,100,150,200,250,300},
  minor y tick num=1,
]
\addplot [KITpurple][line width=1pt] table {deltap_raw.dat};
      \usetikzlibrary {arrows.meta}
 \draw[-{Stealth[black]}] (2.15,125)   -- (1.25,125);
 \draw[-{Stealth[black]}] (3.05,125)   -- (3.95,125);\label{deltapline}

 \addplot [KITpurple][line width=0.6pt,densely dashed] table {deltapan_raw.dat};\label{deltapanline}

% \addplot+[
%     only marks,
%     mark=triangle,
%     mark options={
%          scale=1.25,
%          draw=KITpurple,
%          rotate=180,
%         },
% ]
%     table {Lennard/deltapan_raw.dat};\label{deltapscattermark}
\addplot+[
    only marks,
    mark=triangle,
    mark options={
         scale=1.5,
         draw=KITpurple,
         rotate=180,
        },
]
    coordinates {(0,300.1)}; \label{stealthdeltapscattermark}
    
  % table[meta=ma]
  % {scattered_example.dat};

% \addplot+[KITgreen]
%     only marks,
%     scatter,
%     mark=halfcircle*,
%     mark size=2.9pt]
% table{Lennard/TMAR_raw.dat};
 
\end{axis}

\begin{axis}[
    width = 0.431\textwidth,
  y axis line style = {KITgreen,line width=0.5pt},
  axis y line*=right,
  ymin=0, ymax=300,
  ylabel=$\overline{T}_\mathrm{MA}$ / \si{\kelvin},
  ylabel style = {KITgreen},
  y tick label style= {KITgreen},
  ytick={0,50,100,150,200,250,300},
  minor y tick num=1,
  xlabel={$t$~/~\SI{}{\day}},
  grid=none,
]
 
\addplot [KITgreen][line width=1pt] table {TMAR_raw.dat};\label{TMARline}

% \addplot[color=KITgreen,only marks,mark=halfcircle*, mark size=5pt] coordinates { (3,100)};

\end{axis}

% \node [anchor=north east,
% draw=black,
% fill=white,
% scale=1
% ]
% (legend) at ($(plot.north east)-(2mm ,2mm)$) 
% {\begin{tabular}{l l}
% \ref{deltapscattermark} &  analytical \\ 
% \ref{deltapline} & numerical \\
% \ref{TMARline} & numerical \\
% \end{tabular}};

\end{tikzpicture}
%}

==> Lennard/lambdavsT.tex <==
\begin{tikzpicture}
\pgfplotsset{
    %scale only axis,
    %scaled x ticks=base 10:3,
    xmin=1.5,
    xmax=100,
    minor x tick num=1,
    grid=major,
    %width = 0.431\textwidth,
    width = 0.431\textwidth,
}
\begin{axis}[ymin=10, ymax=300000,
  xmode=log,
  ymode=log,
  %scaled ytick=true,
  ytick={10,100,1000,10000,100000,1000000}, ytick align=outside, ytick pos=left,
  %log ticks with fixed point, % muss fuer Nutzer gesteuerte Ticks hinzugefuegt werden
  %scaled xtick=false, % keine Notation mit 10^x
  %xtick={2,10,100}, xtick align=outside, xtick pos=left,
  %xlabel=Days,
  x tick label style={major tick length=0pt},
  xticklabels=\empty,
  ylabel={$\lambda~/~\si{\watt\per\meter\per\kelvin}$},
  legend pos=south east,
    xminorgrids=true,
    minor grid style={line width=.3pt,draw=gray!50, densely dotted},
    yminorgrids=true,  
  legend style={draw=none,cells={align=left}},
  legend cell align={left}
  ]

\addplot [KITblue][line width=0.75pt] table {4He_raw.dat};\label{curve:4He}
%\addlegendentry{\textsuperscript{4}He at design conditions \cite{sato2006},\cite{HEPAK}}
%\addlegendentry{$\dot{q}=\SI{9.2}{\kilo\watt\per\meter\squared}$\\
%$p=\SI{1.2}{bar(a)}$\\
%$d_\mathrm{h}=\SI{4.5}{\milli\meter}$}

\addplot [KITmaygreen][line width=0.75pt, dashed, densely dashed] table [x=x, y=y,y error=error, col sep=comma]{6NAl_raw.dat};\label{curve:6NAl}
%\addlegendentry{6N-Aluminum \cite{Cryocomp}}

\addplot+[
  KITorange, mark options={KITorange, scale=1.0},
  mark=triangle*,
  smooth, 
  error bars/.cd, 
    y fixed,
    y dir=both, 
    y explicit
] table [x=x, y=y,y error=error, col sep=comma] {Sp_raw.dat};
\label{curve:Sphighpure}
%\addlegendentry{Sapphire, high purity \cite{TPRC2}}

    \addplot+[
    only marks,
    mark=triangle,
    mark options={
         scale=1.0,
         draw=KITorange,
        },
]
    table {SpKAGRA_raw.dat};\label{scatterplot:SpKAGRA}
    %\addlegendentry{Sapphire, single crystal \cite{Khalaidovski_2014}}
  
\addplot+[
  KITpurple, mark options={KITpurple, scale=0.75},
  smooth, 
  mark=square*,
  error bars/.cd, 
    y fixed,
    y dir=both, 
    y explicit
] table [x=x, y=y,y error=error, col sep=comma] {Si_raw.dat};
\label{curve:Sihighpure}
%\addlegendentry{Silicon, high purity \cite{TPRC}}

\addplot[
    only marks,
    mark=square,
    mark options={
         scale=0.75,
         % fill=KITgreen!80!KITgreen,
         draw=KITpurple,
        },
    %scatter,
    % mark=halfcircle*,
    % mark color = KITgreen,
    % mark size=2.9pt
]
    table {SiTravasso_raw.dat};\label{scatterplot:SiTravasso}
    %\addlegendentry{Silicon, single crystal fibers \cite{FlavioSiSuspensions}  }

%\legend{} %hides legend!!

\end{axis}


\begin{axis}[ymin=10, ymax=300000, %additional axis, otherwise wrong notation at x-Labels
  xmode=log,
  ymode=log,
  yticklabels=\empty,
  log ticks with fixed point, % muss fuer Nutzer gesteuerte Ticks hinzugefuegt werden
  %scaled xtick=false, % keine Notation mit 10^x
  xtick={2,10,100}, xtick align=outside, xtick pos=left,
  xlabel={$T~/~\si{\kelvin}$},
  grid=none,
  legend style={draw=none}]
 
  \end{axis}
  
%\begin{spacing}{0.5}
\node at (2.8,4.5)[draw=none,align=left] {%\colorbox{white}{
$p=\SI{1.2}{bar(a)}$,
%}
\\
%\colorbox{white}{
$\dot{q}=\SI{9.2}{\kilo\watt\per\meter\squared}$, $d_\mathrm{h}=\SI{5.8}{\milli\meter}$
%}
%\colorbox{white}{
%}
};
%\end{spacing}
  
\end{tikzpicture}

==> TMAR_deltap_plot.tex <==
%\resizebox{\columnwidth}{!}{%
%\pgfplotsset{width=242.25pt}
\begin{tikzpicture}
\pgfplotsset{
    %scale only axis,
    %scaled x ticks=base 10:3,
    xmin=0,
    xmax=5,
    minor x tick num=1,
    grid=major,
    width = 0.431\textwidth,
}

\begin{axis}[
    width = 0.431\textwidth,
  y axis line style = {KITpurple},
  axis y line*=left,
  axis x line=none,
  ymin=0, ymax=300,
  ylabel=$\Delta p_\mathrm{ma}$ / \SI{}{\milli\bar},
  ylabel style = {KITpurple},
  y tick label style= {KITpurple},
  ytick={0,50,100,150,200,250,300},
  minor y tick num=1,
]
\addplot [KITpurple][line width=1pt] table {deltap_raw.dat};
      \usetikzlibrary {arrows.meta}
 \draw[-{Stealth[black]}] (2.15,125)   -- (1.25,125);
 \draw[-{Stealth[black]}] (3.05,125)   -- (3.95,125);
\end{axis}

\begin{axis}[
    width = 0.431\textwidth,
  y axis line style = {KITgreen},
  axis y line*=right,
  ymin=0, ymax=300,
  ylabel=$\overline{T}_\mathrm{MAR}$ / \si{\kelvin},
  ylabel style = {KITgreen},
  y tick label style= {KITgreen},
  ytick={0,50,100,150,200,250,300},
  minor y tick num=1,
  xlabel={$t$~/~\SI{}{\day}},
]
 
\addplot [KITgreen][line width=1pt] table {TMAR_raw.dat};

\end{axis}

\end{tikzpicture}
%}

==> TTM_plot.tex <==
%\resizebox{\columnwidth}{!}{%
%\pgfplotsset{width=242.25pt}
\usetikzlibrary{calc}

\begin{tikzpicture}
\pgfplotsset{
    %scale only axis,
    %scaled x ticks=base 10:3,
    xmin=0,
    xmax=15,
    minor x tick num=2,
    grid=major,
    width = 0.431\textwidth,
}

\begin{axis}[
    width = 0.431\textwidth,
  %y axis line style = {KITpurple},
  %axis y line=both,
  %axis x line=none,
  ymin=0, ymax=300,
  ylabel=$\overline{T}_\mathrm{MI}~/~\si{\kelvin}$,
  xlabel={$t~/~\si{\day}$},
  %ylabel style = {KITpurple},
  %y tick label style= {KITpurple},
  ytick={0,50,100,150,200,250,300},
  minor y tick num=1,
  %xtick={0,3,6,9,12,15}, 
  xtick distance = 3,
  xtick align=inside,
  %xtick pos=left,
]
\addplot [KITblue][line width=1pt] table {TTM_raw.dat};

\addplot [Gray50][line width=0.75pt, dashed] coordinates {(5.150462963,-1) (5.150462963,301)};
 \usetikzlibrary {arrows.meta};
 % \draw[-{stealth[Gray70]}][Gray70, line width=0.65pt] (3.9,245)   -- (2.3,245);
 % \draw[-{stealth[Gray70]}][Gray70, line width=0.65pt] (6.4,245)   -- (8.0,245);
 % \draw[-][Gray70, line width=0.65pt, densely dotted] (5.4,245)   -- (6.4,245);
 % \draw[-][Gray70, line width=0.65pt, densely dotted] (4.9,245)   -- (3.9,245);
 \draw[-{stealth[Gray70]}][Gray70, line width=0.65pt, densely dotted] (3.3,245)   -- (4.9,245);
 \draw[-{stealth[Gray70]}][Gray70, line width=0.65pt] (6.7,245)   -- (8.3,245);
 \draw[-][Gray70, line width=0.65pt, densely dotted] (5.4,245)   -- (6.7,245);
 \draw[-][Gray70, line width=0.65pt] (2.0,245)   -- (3.3,245); 

\end{axis}

\node at (1.33,3.73)[draw=none,align=right,Gray70] {%\colorbox{white}{
thermal\\radiation%}
};
\node at (3.0,3.883)[draw=none,align=left,Gray70] {%\colorbox{white}{
He-cooling%}
};

\end{tikzpicture}
%}
